One Model, Two Modes: Joint Safety Alignment for Hybrid-Thinking Vision-Language Models

Vision-language models (VLMs) now serve a wide range of multimodal tasks, which differ in how much reasoning they require. To balance performance and speed, recent hybrid-thinking VLMs let users switch a single model between a Thinking (ON) and a Non-Thinking (OFF) mode. However, this mode-switching capability reveals a new safety disparity: across three representative models, the ON mode is consistently more vulnerable, 24.7%-30.8% of harmful inputs yield conflicting safety outcomes across modes, and reasoning traces may contain harmful content even when final responses are safe. Since users can invoke either mode, ensuring the safety of hybrid-thinking VLMs requires aligning both modes, yet existing methods primarily address direct-answer or reasoning models separately. To address this gap, we formalize four criteria for aligning both modes and propose DuoAlign, the first joint safety alignment framework tailored to hybrid-thinking VLMs. DuoAlign samples paired responses from both modes, scores final answers and complete ON outputs with separate trace-aware rewards, and couples the two modes on a shared advantage scale, using OFF as an in-model reference for ON whenever OFF is safer. Evaluated on three models against seven baselines, DuoAlign achieves the highest dual-mode safety-helpfulness harmonic mean on the challenging USB-Hard benchmark, improving it by 14.5-19.2 percentage points (pp) over the base models. It further reduces the cross-mode attack success rate (ASR) gap from 14.3-21.8 to 2.8-3.8 pp while preserving reasoning and general capabilities.

==> sec/2_Related_Work.tex <==
% \section{Related Work}

% \subsection{Vision Language Models}

% \subsection{Reinforcement Learning}

% \subsection{Safety Alignment}
